Study and Design of Reconfigurable Intelligent Surfaces

In this thesis, we introduce the fundamental equations behind the estimation of the link budget in a communications channel, highlighting the key limitations of conventional systems. Furthermore, we investigate the use of reconfigurable intelligent surfaces as a modern method of overcoming obstruction losses, while making use of numerical methods and computational electromagnetics to understand its physical mechanism and probe its theory of operation. Additionally, a preprint on computational geometry is presented, applicable to the field of computational electromagnetics, enabling the simulation of systems such as reconfigurable intelligent surfaces using open-source tools. Lastly, we provide a tool for the physical optimization of radio-frequency networks, based on mathematical programming. Such a tool may be used for the optimization of reconfigurable intelligent surfaces, ultimately improving the communication channel between a transmitter and receiver.

==> core/approval.tex <==
\section*{Approval}

The thesis/project titled “Predicting a T20 Cricket Match Result While The Match is in Progress” submitted by 
\begin{enumerate}
  \item Student Name (Student ID)
  \item Student Name (Student ID)
  \item Student Name (Student ID) 
  \item Student Name (Student ID)
\end{enumerate}

Of Summer, 2015 has been accepted as satisfactory in partial fulfillment of the requirement for the degree of B.Sc. in Computer Science on August 23, 2015. 

\vspace{0.5cm}
\textbf{Examining Committee:}

\vspace{1cm}

Supervisor:\\
(Member)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Name of Supervisor} ~\\ \centerline{Senior Lecturer}~\\ \centerline{Department}~\\ \centerline{Institution} } \hspace{1cm} 
1\end{center}

Program Coordinator:\\
(Member)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Name of Program Coordinator} ~\\ \centerline{Designation}~\\ \centerline{Department}~\\ \centerline{Brac University} } \hspace{1cm} 
\end{center}

Head of Department:\\
(Chair)
\begin{center}
    \hspace{7cm} \wildcard{\centerline{Name of Head of Department} ~\\ \centerline{Designation}~\\ \centerline{Department of Computer Science and Engineering }~\\ \centerline{Brac University} } \hspace{1cm} 
\end{center}

\pagebreak

==> core/declaration.tex <==
% Following command is used to created grouped signature line for Four Authors
\newcommand*\wildcard[2][6cm]{\vspace{2cm}\parbox{#1}{\hrulefill\par#2}} 

% A "parbox{}{}" is a box whose contents are created in paragraph mode. 
% "hrulefill{} to chance thickness of underline"

\section*{Declaration}

It is hereby declared that

\begin{enumerate} % begin{enumerate} function to create numbered list
  \item The thesis submitted is my own original work while completing the degree at the University of Piraeus.
  \item The thesis does not contain material previously published or written by a third party, except where this is appropriately cited through full and accurate referencing.
  \item The thesis does not contain material which has been accepted, or submitted, for any other degree or diploma at a university or other institution.
  \item All main sources of help have been acknowledged.
\end{enumerate}

\vspace{1cm}
\textbf{Student’s Full Name \& Signature:} % Testbf{} for Bold

\begingroup

    \begin{center}
        \wildcard{\centerline{Student Name} ~\\ \centerline{Student ID}} % "centerline{}" to center line
        \hspace{2cm} % "hspace{}" for Blank Horizontal space
        \wildcard{\centerline{Student Name} ~\\ \centerline{Student ID} }
        \wildcard{\centerline{Student Name} ~\\ \centerline{Student ID} }
        \hspace{2cm}
        \wildcard{\centerline{Student Name} ~\\ \centerline{Student ID} }
    \end{center}

\endgroup


\pagebreak







==> core/ethics_statement.tex <==
\section*{Ethics Statement (Optional)}
This is optional, if you don't have an ethics statement then omit this page
\pagebreak
